Tracing Properties of UML and OCL Models with Maude

The starting point of this paper is a system described in form of a UML class diagram where system states are characterized by OCL invariants and system transitions are defined by OCL pre- and postconditions. The aim of our approach is to assist the developer in learning about the consequences of the described system states and transitions and about the formal implications of the properties that are explicitly given. We propose to draw conclusions about the stated constraints by translating the UML and OCL model into the algebraic specification language and system Maude, which is based on rewrite logic. We will concentrate in this paper on employing Maude's capabilities for state search. Maude's state search offers the possibility to describe a start configuration of the system and then explore all configurations reachable by rewriting. The search can be adjusted by formulating requirements for the allowed states and the allowed transitions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{81}
\providecommand{\publicationstatus}{Francisco Dur\'an and Vlad Rusu (Eds.):\\
Second International Workshop on Algebraic Methods\\
in Model-Based Software Engineering 2011 (AMMSE'11)\\
EPTCS 56, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.56.6}{10.4204/EPTCS.56.6}}
\pdfoutput=1

